Realisability of Pomsets via Communicating Automata

Pomsets are a model of concurrent computations introduced by Pratt. They can provide a syntax-oblivious description of semantics of coordination models based on asynchronous message-passing, such as Message Sequence Charts (MSCs). In this paper, we study conditions that ensure a specification expressed as a set of pomsets can be faithfully realised via communicating automata. Our main contributions are (i) the definition of a realisability condition accounting for termination soundness, (ii) conditions for global specifications with "multi-threaded" participants, and (iii) the definition of realisability conditions that can be decided directly over pomsets. A positive by-product of our approach is the efficiency gain in the verification of the realisability conditions obtained when restricting to specific classes of choreographies characterisable in term of behavioural types.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{M. Bartoletti and S. Knight (Eds.):\\ 11th Interaction and Concurrency Experience (ICE 2018)\\
EPTCS 279, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.279.6}{10.4204/EPTCS.279.6}}
\pdfoutput=1

